GPyTorch: Blackbox Matrix-Matrix Gaussian Process Inference with GPU Acceleration

Despite advances in scalable models, the inference tools used for Gaussian processes (GPs) have yet to fully capitalize on developments in computing hardware. We present an efficient and general approach to GP inference based on Blackbox Matrix-Matrix multiplication (BBMM). BBMM inference uses a modified batched version of the conjugate gradients algorithm to derive all terms for training and inference in a single call. BBMM reduces the asymptotic complexity of exact GP inference from $O(n^3)$ to $O(n^2)$. Adapting this algorithm to scalable approximations and complex GP models simply requires a routine for efficient matrix-matrix multiplication with the kernel and its derivative. In addition, BBMM uses a specialized preconditioner to substantially speed up convergence. In experiments we show that BBMM effectively uses GPU hardware to dramatically accelerate both exact GP inference and scalable approximations. Additionally, we provide GPyTorch, a software platform for scalable GP inference via BBMM, built on PyTorch.

==> complexity_table.tex <==
\begin{table*}[t!]
  \caption{
    Asymptotic complexities of matrix-vector multiplications (MVMs),
    computing the pivoted-Cholesky preconditioner (PC-precond.),
    and performing inference.
    ($n$ data points, $m$ inducing points, $p$ iterations of CG, and $t$ initial probe vectors for Lanczos.)
    \jrg{My vote is to remove the preconditioner from the running times -- the complexities are just too complicated imo}
    \label{tab:running_times}
  }
  \vspace{0.5ex}
  \centering
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{ |c||c|c||c|c||c| }
      \hline
      \
      \multirow{2}*{\bf Method}
      & \multirow{2}*{\bf One MVM}
      & {\bf PC}
      & {\bf MVM-based inference}
      & {\bf MVM-based inference}
      & \multirow{2}*{\bf Cholesky-based inference}
      \\
      &
      & {\bf precond.}
      & (no precond.)
      & (with PC-precond.)
      &
      \\
      \hhline{|=#=|=#=|=#=|}
      Standard GP
      & $\bigo{n^2}$
      & $\bigo{n k^2}$
      & $\bigo{t p (n^2)}$
      & $\bigo{t p (n^2) + t n k^2}$
      & $\bigo{n^3}$
      \\
      SGPR
      & $\bigo{n m + m^2}$
      & $\bigo{n m k^2}$
      & $\bigo{t p (n m + m^2)}$
      & $\bigo{t p (n m + m^2) + n m k^2}$
      & $\bigo{n m^2 + m^3}$
      \\
      SKI
      & $\bigo{n + m \log m}$
      & $\bigo{n k^2}$
      & $\bigo{t p (n + m \log m)}$
      & $\bigo{t p (n + m \log m) + t n k^2}$
      & --
      \\
      \hline
    \end{tabular}
  }
  \vspace{-2ex}
\end{table*}


==> theory.tex <==
%!TEX root=main.tex
\paragraph{Theoretical analysis of CG convergence.}
By leveraging analysis from \cite{harbrecht2012low}, we can show that for RBF kernels the condition number of the preconditioned $\trainK$ matrix decreases exponentially with the rank $k$ of $L_k$.
We begin by restating \cite{harbrecht2012low} primary convergence result.
%
\begin{theorem}[\citet{harbrecht2012low}]
If the eigenvalues of an $n \times n$ positive definite and symmetric matrix $K_{XX}$ satisfy $4^{k}\lambda_{k} \lesssim \exp(-bk)$ for some $b>0$, then
the rank $k$ pivoted Cholesky decomposition $P_{k}$ satisfies $\textrm{Tr}(K_{XX} - P_{k}) \lesssim n\exp(-bk)$.
\label{thm:harbrecht}
\end{theorem}
Intuitively, if the eigenvalues of a matrix decay very quickly (exponentially), then it is very easy to approximate with a low rank matrix, and the pivoted Cholesky algorithm rapidly constructs such a matrix.
While there has been an enormous amount of work understanding the eigenvalue distributions of kernel functions \jrg{cite cite cite}, in this paper we prove the following useful bound on the eigenvalue distribution of univariate RBF kernel matrices:
%
\begin{theorem}
\label{thm:eigenvalue_bound}
Given $\bu_1,...,\bu_n \in [0, 1]$, the RBF kernel matrix $K_{XX} \in \mathbb{R}^{n \times n}$ with $K_{ij} = \exp \left(-\gamma(x_i - x_j)^{2}\right)$ has eigenvalues bounded by:
\begin{equation*}
    \lambda_{2l+1} \leq
    2n e^{-\gamma/4} I_{l+1}(\gamma/4) \sim
    \frac{2n e^{-\gamma/4}}{\sqrt{\pi\gamma}}
    \left( \frac{e\gamma}{8(l+1)} \right)^{l+1}
\end{equation*}
where $I_j$ denotes the modified Bessel function of the first kind with parameter $j$.
\end{theorem}
%
Thus, the eigenvalues of an RBF kernel matrix $K_{XX}$ decay \emph{super-exponentially}, and so the bound given by \autoref{thm:harbrecht} applies.
These two theorems together let us argue for the theoretical soundness of the pivoted Cholesky decomposition as a preconditioner.
To bound the condition number of the matrix $\trainP^{-1} \trainK$, we begin bounding the difference between a linear solve with the $\trainP$ and the full matrix $\trainK$.
%
\begin{theorem}
Let $\by$ be any vector, and let $\bu^{*} = \trainK^{-1}\by$ and $\tilde{\bu} = \trainP_{k}^{-1}\by$, where $\trainP_{k}=L_{k} L_K^\top + \sigma^{2}I$ and $L_{k} L_k^\top$ is the rank $k$ pivoted Cholesky decomposition of $K_{XX}$.
There exists some $b>0$ so that $\frac{\Vert \bu^{*} - \tilde{\bu}\Vert_{2}}{\Vert\bu^{*}\Vert_{2}} \lesssim \frac{n\exp(-bk)}{\sigma}$.
\end{theorem}
%
Intuitively, this theorem states that the pivoted Cholesky preconditioner converges rapidly to $\trainK^{-1}$, which is the optimal preconditioner in terms of the number of CG iterations.
Athe norm $\Vert \trainP_{k}^{-1} - \trainK^{-1} \Vert$ decreases, the convergence rate of CG increases.
Finally, to explicitly relate the above theorem to the rate of convergence of CG, we can prove the following bound on the condition number:
%
\begin{theorem}
  \label{thm:condition_number}
  Let $P_{k}$ be the rank $k$ pivoted Cholesky decomposition of $K$, and let $\trainP_{k} = P_{k} + \sigma^{2}I$. Then the condition number $\kappa(\trainP^{-1}\trainK)$ satisfies the following inequality:
  \begin{equation}
    \kappa(\trainP_{k}^{-1}\trainK) \triangleq \Vert \trainP_{k}^{-1}\trainK \Vert_{2} \Vert \trainK^{-1}\trainP_{k} \Vert_{2} \leq 1 + \bigo{\frac{n\exp(-bk)}{\sigma}}.
  \end{equation}
\end{theorem}
%
This last result lets us directly speak about the impact of our preconditioner on the convergence of conjugate gradients.
In particular, when solving a system $\trainP_{k}^{-1}\trainK\bu = \trainP_{k}^{-1}\by$, the solution $\bu_{p}$ after $p$ iterations of conjugate gradients in exact arithmetic is related to the optimal solution $\bu^{*}$ by the following inequality involving the condition number \jrg{cite}:
%
\begin{equation}
  \begin{aligned}
  \Vert \trainK^{-1} y - \bu_{k} \Vert_{A}
  &\leq 2 \left( \left( {\sqrt{\kappa\left(\trainP_{k}^{-1}\trainK\right)} - 1} \right) / \left( {\sqrt{\kappa\left(\trainP_{k}^{-1}\trainK\right)} + 1} \right) \right)^{p}\Vert \trainK^{*}\y - \bu_{0} \Vert_{A}
  \\
  &\leq 2 \left(\frac{1}{2 + \bigo{n e^{-kb/2} / \sigma}}\right)^{p}\Vert \trainK^{-1} y - \bu_{0} \Vert_{A}
\end{aligned}
\end{equation}
%
Thus, \autoref{thm:condition_number} implies that the pivoted Cholesky preconditioner exponentially improves the rate of convergence as $k$ increases.

